Search for supersymmetry in events with four or more leptons in $\sqrt{s}=13$ TeV $pp$ collisions with ATLAS

Results from a search for supersymmetry in events with four or more charged leptons (electrons, muons and taus) are presented. The analysis uses a data sample corresponding to 36.1 fb$^{-1}$ of proton-proton collisions delivered by the Large Hadron Collider at $\sqrt{s}=13$ TeV and recorded by the ATLAS detector. Four-lepton signal regions with up to two hadronically decaying taus are designed to target a range of supersymmetric scenarios that can be either enriched in or depleted of events involving the production and decay of a $Z$ boson. Data yields are consistent with Standard Model expectations and results are used to set upper limits on the event yields from processes beyond the Standard Model. Exclusion limits are set at the 95% confidence level in simplified models of General Gauge Mediated supersymmetry, where higgsino masses are excluded up to 295 GeV. In $R$-parity-violating simplified models with decays of the lightest supersymmetric particle to charged leptons, lower limits of 1.46 TeV, 1.06 TeV, and 2.25 TeV are placed on wino, slepton and gluino masses, respectively.

==> acknowledgements/Makefile <==
# Makefile for creating ATLAS Acknowledegments

TEXLIVE  = 2016
PDFLATEX = pdflatex
BIBTEX   = biber

BASENAME = Acknowledgements-main

.PHONY: clean cleanpdf

run_pdflatex: $(BASENAME).pdf
	@echo "Made $<"

# Change TeX Live version
texlive: $(BASENAME).tex
	if [ $(TEXLIVE) -ge 2007 -a $(TEXLIVE) -lt 2100 ]; then \
	  echo "Changing texlive value in $<"; \
	  sed -i'.bak' 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' $<; \
	else echo "Invalid value for TEXLIVE: $(TEXLIVE)"; fi; \

# Change biblatex backend
bibtex: $(BASENAME).tex
	if [ $(BIBTEX) = 'biber' -o $(BIBTEX) = 'bibtex' ]; then \
	  echo "Changing biblatex backend in $<"; \
	  sed -i'.bak' -e 's/backend=biber/backend=$(BIBTEX)/' -e 's/backend=bibtex/backend=$(BIBTEX)/' $<; \
	else echo "Invalid value for BIBTEX: $(BIBTEX)"; fi; \

# Standard LaTeX targets
$(BASENAME).pdf: $(BASENAME).tex
	$(PDFLATEX) $<
	-$(BIBTEX)  $(basename $<)
	$(PDFLATEX) $<
	$(PDFLATEX) $<

%.bbl: %.tex *.bib
	$(PDFLATEX) $*
	$(BIBTEX) $*

clean:
	-rm *.dvi *.toc *.aux *.log *.out *.blg *.bbl *.bcf *-blx.bib \
	 *.run.xml *.synctex.gz *~ *.fls *.fdb_latexmk .*.lb spellTmp 

cleanpdf:
	-rm $(BASENAME).pdf

cleanall: clean cleanpdf


==> paper_aux.tex <==
\clearpage
\newpage
\section*{Auxiliary Material} 



\begin{sidewaystable}[h]{\footnotesize
\begin{center}
\begin{tabular}{l | l l l l l l l}
%
\toprule
Region 
%
& wino NLSP $\lambda_{12k}$ 
& wino NLSP $\lambda_{i33}$
%
& $\tilde{l}_L/\tilde{\nu}$ NLSP $\lambda_{12k}$  
& $\tilde{l}_L/\tilde{\nu}$ NLSP $\lambda_{i33}$ 
%
& $\tilde{g}$ NLSP $\lambda_{12k}$ 
& $\tilde{g}$ NLSP $\lambda_{i33}$ 
%
& GGM higgsino \\
\toprule
SR0A & 			& 		& 	 	&		& 		&		& \\
SR0B & \textbullet	& \textbullet	& \textbullet	& \textbullet	& \textbullet 	&\textbullet	& \\
SR0C &			& 		& 		& 		& 		&		&\textbullet \\
SR0D &			&		& 		& 		& 		&		&\textbullet \\
SR1  & 			& \textbullet	&	 	& \textbullet	& 		&\textbullet	& \\
SR2  &			& \textbullet	&	 	& \textbullet	& 		&\textbullet	& \\
\bottomrule
%
\end{tabular}
\end{center}
\caption{Summary of the best expected signal region per signal model. 
This mapping is being used for the final combined exclusion limits.
SR0A typically contributes only in the very low mass regime for all models in the combination of the best expected exclusion limits.
Thus SR0A does not have a significant impact on the calculation of the upper limits on the signal cross section at higher signal masses.
}
\label{tb:best_expected_all} 
}
\end{sidewaystable}


%VVz SR0A
\begin{figure}[h]
 \centering
 \subfloat[][RPV wino \Wboson/\Zboson NLSP $\LLE 12k$ - SR0A]{
 \includegraphics[width=0.75\textwidth]{../figures/limitPlots/Jan/limit_VVz_version310118up_SR0A_LLE12k_OBS} %LLE12k
 } 
 \\
 \subfloat[][RPV wino \Wboson/\Zboson NLSP $\LLE i33$ - SR0A+SR1+SR2]{
 \includegraphics[width=0.75\textwidth]{../figures/limitPlots/Jan/limit_VVz_version310118up_SR0A+_LLEi33_OBS} %LLEi33
 }
 \caption{
 Observed and expected exclusion limits on the $\chinoonepm/\ninotwo$  masses in the context of the wino \Wboson/\Zboson RPV scenario with $\LLE 12k$ (top) and $\LLE i33$  (bottom) couplings.
 The signal region used to obtain the limits is SR0A for the $\LLE 12k$ case, and the combination of SR0A, SR1 and SR2 for the $\LLE i33$ one.
 All limits are computed at 95\% CL. 
 The dotted lines around the observed limit illustrate the change in the observed limit as the nominal signal cross-section is scaled up and down by the theoretical uncertainty. 
 The contours of the band around the expected limit are the $\pm 1~\sigma$ results, including all uncertainties except the theoretical ones on the signal cross-section. 
 The diagonal lines indicate the kinematic limit for the decays in this particular scenario. 
 The grey numbers represent the 95\% CL upper limits on the production cross-section (in $\mathrm{fb}$) 
 obtained using the signal efficiency and acceptance specific to this model.
 }
 \label{fig:upper_limits_VVz_A}
\end{figure}


%VVz SR0B+
\begin{figure}[h]
 \centering
 \subfloat[][RPV wino \Wboson/\Zboson NLSP $\LLE 12k$ - SR0B]{
 \includegraphics[width=0.75\textwidth]{../figures/limitPlots/Jan/limit_VVz_version310118up_SR0B_LLE12k_OBS}%LLE12k
 } 
 \\
 \subfloat[][RPV wino \Wboson/\Zboson NLSP $\LLE i33$ - SR0B+SR1+SR2]{
 \includegraphics[width=0.75\textwidth]{../figures/limitPlots/Jan/limit_VVz_version310118up_SR0B+_LLEi33_OBS}%LLEi33
 }
 \caption{
 Observed and expected exclusion limits on the $\chinoonepm/\ninotwo$  masses in the context of the wino \Wboson/\Zboson RPV scenario with 
 $\LLE 12k$ (top) and $\LLE i33$  (bottom) couplings.
 The signal region used to obtain the limits is SR0B for the $\LLE 12k$ case, and the combination of SR0B, SR1 and SR2 for the $\LLE i33$ one.
 All limits are computed at 95\% CL. 
 The dotted lines around the observed limit illustrate the change in the observed limit as the nominal signal cross-section is scaled up and down by the theoretical uncertainty. 
 The contours of the band around the expected limit are the $\pm 1~\sigma$ results, including all uncertainties except the theoretical ones on the signal cross-section. 
 The diagonal lines indicate the kinematic limit for the decays in this particular scenario. 
 The grey numbers represent the 95\% CL upper limits on production cross-section (in $\mathrm{fb}$) 
 obtained using the signal efficiency and acceptance specific to this model.
 }
 \label{fig:upper_limits_VVz_B}
\end{figure}


%VVh SR0A
\begin{figure}[h]
 \centering
 \subfloat[][RPV wino \Wboson/\Higgs NLSP $\LLE 12k$ - SR0A]{
 \includegraphics[width=0.75\textwidth]{../figures/limitPlots/Jan/limit_VVh_version310118up_SR0A_LLE12k_OBS} %LLE12k
 } 
 \\
 \subfloat[][RPV wino \Wboson/\Higgs NLSP $\LLE i33$ - SR0A+SR1+SR2]{
 \includegraphics[width=0.75\textwidth]{../figures/limitPlots/Jan/limit_VVh_version310118up_SR0A+_LLEi33_OBS} %LLEi33
 }
 \caption{
 Observed and expected exclusion limits on the $\chinoonepm/\ninotwo$  masses in the context of the wino \Wboson/\Higgs RPV scenario with $\LLE 12k$ (top) and $\LLE i33$  (bottom) couplings.
 The signal region used to obtain the limits is SR0A for the $\LLE 12k$ case, and the combination of SR0A, SR1 and SR2 for the $\LLE i33$ one.
 All limits are computed at 95\% CL. 
 The dotted lines around the observed limit illustrate the change in the observed limit as the nominal signal cross-section is scaled up and down by the theoretical uncertainty. 
 The contours of the band around the expected limit are the $\pm 1~\sigma$ results, including all uncertainties except the theoretical ones on the signal cross-section. 
 The diagonal lines indicate the kinematic limit for the decays in this particular scenario. 
 The grey numbers represent the 95\% CL upper limits on the production cross-section (in $\mathrm{fb}$) 
 obtained using the signal efficiency and acceptance specific to this model.
 }
 \label{fig:upper_limits_VVz_A}
\end{figure}


%VVh SR0B+
\begin{figure}[h]
 \centering
 \subfloat[][RPV wino \Wboson/\Higgs NLSP $\LLE 12k$ - SR0B]{
 \includegraphics[width=0.75\textwidth]{../figures/limitPlots/Jan/limit_VVh_version310118up_SR0B_LLE12k_OBS}%LLE12k
 } 
 \\
 \subfloat[][RPV wino \Wboson/\Higgs NLSP $\LLE i33$ - SR0B+SR1+SR2]{
 \includegraphics[width=0.75\textwidth]{../figures/limitPlots/Jan/limit_VVh_version310118up_SR0B+_LLEi33_OBS}%LLEi33
 }
 \caption{
 Observed and expected exclusion limits on the $\chinoonepm/\ninotwo$  masses in the context of the wino \Wboson/\Higgs RPV scenario with 
 $\LLE 12k$ (top) and $\LLE i33$  (bottom) couplings.
 The signal region used to obtain the limits is SR0B for the $\LLE 12k$ case, and the combination of SR0B, SR1 and SR2 for the $\LLE i33$ one.
 All limits are computed at 95\% CL. 
 The dotted lines around the observed limit illustrate the change in the observed limit as the nominal signal cross-section is scaled up and down by the theoretical uncertainty. 
 The contours of the band around the expected limit are the $\pm 1~\sigma$ results, including all uncertainties except the theoretical ones on the signal cross-section. 
 The diagonal lines indicate the kinematic limit for the decays in this particular scenario. 
 The grey numbers represent the 95\% CL upper limits on production cross-section (in $\mathrm{fb}$) 
 obtained using the signal efficiency and acceptance specific to this model.
 }
 \label{fig:upper_limits_VVz_B}
\end{figure}

% LH LV SR0A
\begin{figure}[h]
 \centering
 \subfloat[][RPV $\sleptonL/\snu$ NLSP $\LLE 12k$ - SR0A]{
 \includegraphics[width=0.75\textwidth]{../figures/limitPlots/Jan/limit_LV_version310118up_SR0A_LLE12k_OBS}
 } 
 \\
 \subfloat[][RPV $\sleptonL/\snu$ NLSP $\LLE i33$ - SR0A+SR1+SR2]{
 \includegraphics[width=0.75\textwidth]{../figures/limitPlots/Jan/limit_LV_version310118up_SR0A+_LLEi33_OBS}
 }
 \caption{
 Observed and expected exclusion limits on the left-handed slepton/sneutrino masses in the context of the wino RPV scenario with $\LLE 12k$ (top) 
 and $\LLE i33$  (bottom) couplings.
 The signal region used to obtain the limits is SR0A for the $\LLE 12k$ case, and the combination of SR0A, SR1 and SR2 for the $\LLE i33$ one.
 All limits are computed at 95\% CL. 
 The dotted lines around the observed limit illustrate the change in the observed limit as the nominal signal cross-section is scaled up and down by the theoretical uncertainty. 
 The contours of the band around the expected limit are the $\pm 1~\sigma$ results, including all uncertainties except the theoretical ones on the signal cross-section. 
 The diagonal lines indicate the kinematic limit for the decays in this particular scenario. 
 The grey numbers represent the 95\% CL upper limits on production cross-section (in $\mathrm{fb}$) 
 obtained using the signal efficiency and acceptance specific to this model.
 }
 \label{fig:upper_limits_LV_A}
\end{figure}


% LH LV SR0B+
\begin{figure}[h]
 \centering
 \subfloat[][RPV $\sleptonL/\snu$ NLSP $\LLE 12k$ - SR0B]{
 \includegraphics[width=0.75\textwidth]{../figures/limitPlots/Jan/limit_LV_version310118up_SR0B_LLE12k_OBS}
 } 
 \\
 \subfloat[][RPV $\sleptonL/\snu$ NLSP $\LLE i33$ - SR0B+SR1+SR2]{
 \includegraphics[width=0.75\textwidth]{../figures/limitPlots/Jan/limit_LV_version310118up_SR0B+_LLEi33_OBS}
 }
 \caption{
 Observed and expected exclusion limits on the left-handed slepton/sneutrino masses in the context of the wino RPV scenario with $\LLE 12k$ (top) 
 and $\LLE i33$  (bottom) couplings.
 The signal region used to obtain the limits is SR0B for the $\LLE 12k$ case, and the combination of SR0B, SR1 and SR2 for the $\LLE i33$ one.
 All limits are computed at 95\% CL. 
 The dotted lines around the observed limit illustrate the change in the observed limit as the nominal signal cross-section is scaled up and down by the theoretical uncertainty. 
 The contours of the band around the expected limit are the $\pm 1~\sigma$ results, including all uncertainties except the theoretical ones on the signal cross-section. 
 The diagonal lines indicate the kinematic limit for the decays in this particular scenario. 
 The grey numbers represent the 95\% CL upper limits on production cross-section (in $\mathrm{fb}$) 
 obtained using the signal efficiency and acceptance specific to this model.
 }
 \label{fig:upper_limits_LV_B}
\end{figure}

% GG SR0A
\begin{figure}[h]
 \centering
 \subfloat[][RPV $\gluino$  NLSP $\LLE 12k$ - SR0A]{
 \includegraphics[width=0.75\textwidth]{../figures/limitPlots/Jan/limit_GG_version310118up_SR0A_LLE12k_OBS}
 } 
 \\
 \subfloat[][RPV $\gluino$  NLSP $\LLE i33$ - SR0A+SR1+SR2]{
 \includegraphics[width=0.75\textwidth]{../figures/limitPlots/Jan/limit_GG_version310118up_SR0A+_LLEi33_OBS}
 }
 \caption{
 Observed and expected exclusion limits on the $\gluino$ masses in the context of the gluino RPV scenario with $\LLE 12k$ (top) 
 and $\LLE i33$  (bottom) couplings.
 The signal region used to obtain the limits is SR0A for the $\LLE 12k$ case, and the combination of SR0A, SR1 and SR2 for the $\LLE i33$ one.
 All limits are computed at 95\% CL. 
 The dotted lines around the observed limit illustrate the change in the observed limit as the nominal signal cross-section is scaled up and down by the theoretical uncertainty. 
 The contours of the band around the expected limit are the $\pm 1~\sigma$ results, including all uncertainties except the theoretical ones on the signal cross-section. 
 The diagonal lines indicate the kinematic limit for the decays in this particular scenario. 
 The grey numbers represent the 95\% CL upper limits on production cross-section (in $\mathrm{fb}$) 
 obtained using the signal efficiency and acceptance specific to this model.
 }
 \label{fig:upper_limits_GG_A}
\end{figure}

% GG SR0B+
\begin{figure}[h]
 \centering
 \subfloat[][RPV $\gluino$  NLSP $\LLE 12k$ - SR0B]{
 \includegraphics[width=0.75\textwidth]{../figures/limitPlots/Jan/limit_GG_version310118up_SR0B_LLE12k_OBS}
 } 
 \\
 \subfloat[][RPV $\gluino$  NLSP $\LLE i33$ - SR0B+SR1+SR2]{
 \includegraphics[width=0.75\textwidth]{../figures/limitPlots/Jan/limit_GG_version310118up_SR0B+_LLEi33_OBS}
 }
 \caption{
 Observed and expected exclusion limits on the $\gluino$ masses in the context of the gluino RPV scenario with $\LLE 12k$ (top) 
 and $\LLE i33$  (bottom) couplings.
 The signal region used to obtain the limits is SR0B for the $\LLE 12k$ case, and the combination of SR0B, SR1 and SR2 for the $\LLE i33$ one.
 All limits are computed at 95\% CL. 
 The dotted lines around the observed limit illustrate the change in the observed limit as the nominal signal cross-section is scaled up and down by the theoretical uncertainty. 
 The contours of the band around the expected limit are the $\pm 1~\sigma$ results, including all uncertainties except the theoretical ones on the signal cross-section. 
 The diagonal lines indicate the kinematic limit for the decays in this particular scenario. 
 The grey numbers represent the 95\% CL upper limits on production cross-section (in $\mathrm{fb}$) 
 obtained using the signal efficiency and acceptance specific to this model.
 }
 \label{fig:upper_limits_GG_B}
\end{figure}


% GGM
\begin{figure}[h]
 \centering
 \subfloat[][GGM higgsino RPC model - SR0C]{
 \includegraphics[width=0.75\textwidth]{../figures/limitPlots/March/limit_GGM_version060318up_SR0C_OBS}
 } 
 \\
 \subfloat[][GGM higgsino RPC model - SR0D]{
 \includegraphics[width=0.75\textwidth]{../figures/limitPlots/March/limit_GGM_version060318up_SR0D_OBS}
 }
 \caption{
 Observed and expected exclusion limits on the $\chinoonepm/\ninotwo/\ninoone$ masses in the context of the higgsino GGM scenario in the SR0C (top) and SR0D (bottom) regions.
 All limits are computed at 95\% CL. 
 The dotted lines around the observed limit illustrate the change in the observed limit as the nominal signal cross-section is scaled up and down by the theoretical uncertainty. 
 The contours of the band around the expected limit are the $\pm 1~\sigma$ results, including all uncertainties except the theoretical ones on the signal cross-section. 
 The diagonal lines indicate the kinematic limit for the decays in this particular scenario. 
 The grey numbers represent the 95\% CL upper limits on production cross-section (in $\mathrm{fb}$) 
 obtained using the signal efficiency and acceptance specific to this model.
 }
 \label{fig:upper_limits_GGM}
\end{figure}

\FloatBarrier

%% done to here figaux_10 is next
% VVz 
\begin{figure}[h]
\begin{center}
\subfloat[][wino \Wboson/\Zboson $\LLE 12k$]{
\includegraphics[width=0.75\textwidth]{../figures/limitPlots/Jan/limit_VVz_version310118_comb_12k_overlay_OBS}
\label{fig:limit_VVz_version310118_comb_12k_overlay_OBS}}\\
\subfloat[][wino \Wboson/\Zboson $\LLE i33$]{
\includegraphics[width=0.75\textwidth]{../figures/limitPlots/Jan/limit_VVz_version310118_comb_i33_overlay_OBS}
\label{fig:limit_VVz_version310118_comb_i33_overlay_OBS}}
\end{center}
\caption{The best expected exclusion power between signal regions at each signal point
as is adopted in the limit calculation of the wino \Wboson/\Zboson model for the \protect\subref{fig:limit_VVz_version310118_comb_12k_overlay_OBS}~$\LLE 12k$  
and \protect\subref{fig:limit_VVz_version310118_comb_i33_overlay_OBS}~$\LLE i33$ couplings.
%
For the $\LLE 12k$ case, the results from SR0B are adopted everywhere in the final exclusion limit contours, 
as is found to be the most powerful signal region among SR0A and SR0B in the majority of the signal grid points of this model.
%
For the $\LLE i33$ case instead, a combination of SR0B + SR1 + SR2  or SR0B + SR1 + SR2 is tested to detect the best expected limit; 
shown on the plot is the region (SR0A or SR0B) which is chosen to provide the best expected limit in combination with SR1 and SR2.
The results from the combination SR0B + SR1 + SR2 are finally adopted everywhere in the final exclusion limit contour since they provide the best expected limit.
}
\label{fig:best_expected_wino_wz}
\end{figure}

% VVz
\begin{figure}[h]
\begin{center}
\subfloat[][wino \Wboson/\Higgs $\LLE 12k$]{
\includegraphics[width=0.75\textwidth]{../figures/limitPlots/Jan/limit_VVh_version310118_comb_12k_overlay_OBS}
\label{fig:limit_VVh_version310118_comb_12k_overlay_OBS}}\\
\subfloat[][wino \Wboson/\Higgs $\LLE i33$]{
\includegraphics[width=0.75\textwidth]{../figures/limitPlots/Jan/limit_VVh_version310118_comb_i33_overlay_OBS}
\label{fig:limit_VVh_version310118_comb_i33_overlay_OBS}}
\end{center}
\caption{The best expected exclusion power between signal regions at each signal point
as is adopted in the limit calculation of the wino \Wboson/\Higgs model for the \protect\subref{fig:limit_VVh_version310118_comb_12k_overlay_OBS}~$\LLE 12k$  
and \protect\subref{fig:limit_VVz_version310118_comb_i33_overlay_OBS}~$\LLE i33$ couplings.
%
For the $\LLE 12k$ case, the results from SR0B are adopted everywhere in the final exclusion limit contours, 
as is found to be the most powerful signal region among SR0A and SR0B in the majority of the signal grid points of this model.
%
For the $\LLE i33$ case instead, a combination of SR0B + SR1 + SR2  or SR0B + SR1 + SR2 is tested to detect the best expected limit; 
shown on the plot is the region (SR0A or SR0B) which is chosen to provide the best expected limit in combination with SR1 and SR2.
The results from the combination SR0B + SR1 + SR2 are finally adopted everywhere in the final exclusion limit contour since they provide the best expected limit.
}
\label{fig:best_expected_wino_wh}
\end{figure}



% LV
\begin{figure}[h]
\begin{center}
\subfloat[][$\sleptonL/\snu$  $\LLE 12k$]{
\includegraphics[width=0.75\textwidth]{../figures/limitPlots/Jan/limit_LV_version310118_comb_12k_overlay_OBS}
\label{fig:limit_LV_version310118_comb_12k_overlay_OBS}
}\\
\subfloat[][$\sleptonL/\snu$  $\LLE i33$]{
\includegraphics[width=0.75\textwidth]{../figures/limitPlots/Jan/limit_LV_version310118_comb_i33_overlay_OBS}
\label{fig:limit_LV_version310118_comb_i33_overlay_OBS}
}
\end{center}
\caption{The best expected exclusion power between signal regions at each signal point
as is adopted in the limit calculation of the slepton/sneutrino model for 
the \protect\subref{fig:limit_LV_version310118_comb_12k_overlay_OBS}~$\LLE 12k$ and \protect\subref{fig:limit_LV_version310118_comb_i33_overlay_OBS}~$\LLE i33$ couplings.
%
For the $\LLE 12k$ case, the results from SR0B are adopted everywhere in the final exclusion limit contours, 
as is found to be the most powerful signal region among SR0A and SR0B in the majority of the signal grid points of this model.
%
For the $\LLE i33$ case instead, a combination of SR0B + SR1 + SR2  or SR0B + SR1 + SR2 is tested to detect the best expected limit; 
shown on the plot is the region (SR0A or SR0B) which is chosen to provide the best expected limit in combination with SR1 and SR2.
The results from the combination SR0B + SR1 + SR2 are finally adopted everywhere in the final exclusion limit contour since they provide the best expected limit.
}
\label{fig:best_expected_slepton}
\end{figure}
% 


% gluino
\begin{figure}[h]
\begin{center}
\subfloat[][gluino $\LLE 12k$]{\includegraphics[width=0.75\textwidth]{../figures/limitPlots/Jan/limit_GG_version310118_comb_12k_overlay_OBS}
\label{fig:limit_GG_version310118_comb_12k_overlay_OBS}}\\
\subfloat[][gluino $\LLE i33$]{\includegraphics[width=0.75\textwidth]{../figures/limitPlots/Jan/limit_GG_version310118_comb_i33_overlay_OBS}
\label{fig:limit_GG_version310118_comb_i33_overlay_OBS}}
\end{center}
\caption{The best expected exclusion power between signal regions at each signal point
as is adopted in the limit calculation of the gluino model for the (a) $\LLE 12k$ (a) and (b) $\LLE i33$ couplings.
%
For the $\LLE 12k$ case, the results from SR0B are adopted everywhere in the final exclusion limit contours, 
as is found to be the most powerful signal region among SR0A and SR0B in the majority of the signal grid points of this model.
%
For the $\LLE i33$ case instead, a combination of SR0B + SR1 + SR2  or SR0B + SR1 + SR2 is tested to detect the best expected limit; 
shown on the plot is the region (SR0A or SR0B) which is chosen to provide the best expected limit in combination with SR1 and SR2.
The results from the combination SR0B + SR1 + SR2 are finally adopted everywhere in the final exclusion limit contour since they provide the best expected limit.
}
\label{fig:best_expected_gluino}
\end{figure}




%GGM
\begin{figure}[h]
 \centering
 \includegraphics[width=0.85\textwidth]{../figures/limitPlots/March/limit_GGM_version060318_comb_overlay_OBS}
 \caption{
 The best expected exclusion power between the overlapping SR0C and SR0D at each signal point
as is adopted in the limit combination of the GGM higgsino model.}
 \label{fig:best_expected_ggm}
\end{figure}

\FloatBarrier

%%%%%%%%%%%%%%%%%%%%%%%%%% Pulls
\begin{figure}[ht]
  \begin{adjustbox}{addcode={ \centering
  \begin{minipage}{\width}}{
 \caption{Comparison of the observed data ($n_{\mathrm obs}$) with the predicted SM background ($n_{\mathrm exp}$) in all validation and signal regions (pulls). 
 The hatched, grey area around the SM prediction includes all uncertainties considered in the analysis.
 The bottom panel shows the difference between data and the predicted SM background divided by the total uncertainty ($\sigma_{\mathrm tot}$).}
  \end{minipage}},rotate=90,center}
   \includegraphics[width=22cm]{../figures/Pulls/histpull_VRSR.eps}
  \label{fig:histpull_VRSR}
  \end{adjustbox}
\end{figure}

\FloatBarrier

%%%%%%%%%%%%%%%%%%%%%%%%%% Histogram Yields

%Feb 2018
\begin{table}[h]{\small
		\centering
		{\renewcommand{\arraystretch}{2}
			\begin{tabular}{lllll|lll}
				\hline
				Component & \multicolumn{6}{c}{Histogram Bin}  \\
				& 7  & 8  & 9  & 10  & 11  & 12  & 13 \\
				\hline
				min $\meff ~[\GeV]$ & 600.0  & 700.0  & 800.0  & 900.0  & 1000.0  & 1100.0  & 1500.0 \\
				max $\meff ~[\GeV]$ & 700.0  & 800.0  & 900.0  & 1000.0  & 1100.0  & 1500.0  & 1900.0 \\
				\hline
				Other & \num{0.0419}  & \num{0.0311}  & \num{0.0253}  & \num{0.0339}  & \num{0.0270}  & \num{0.0215}  & \num{0.0054} \\
				VVV & \num{0.1876}  & \num{0.0840}  & \num{0.0812}  & \num{0.0487}  & \num{0.0781}  & \num{0.0325}  & \num{0.0037} \\
				Higgs & \num{0.3879}  & \num{0.3078}  & \num{0.1992}  & \num{0.0960}  & \num{0.0678}  & \num{0.0273}  & \num{0.0026} \\
				$t\bar{t}Z$ & \num{0.4671}  & \num{0.3551}  & \num{0.2564}  & \num{0.1563}  & \num{0.1143}  & \num{0.0503}  & \num{0.0112} \\
				ZZ & \num{0.9816}  & \num{0.6247}  & \num{0.3256}  & \num{0.2729}  & \num{0.1896}  & \num{0.0499}  & \num{0.0211} \\
				Reducible & \num{0.9370}  & \num{0.4308}  & \num{0.5298}  & \num{0.5823}  & \num{0.2240}  & \num{0.0000}  & \num{0.0000} \\
				Stat. $\otimes$ Syst. & ${}^{+\num{1.0888}}_{-\num{1.0736}}$ & ${}^{+\num{0.9458}}_{-\num{0.9270}}$ & ${}^{+\num{0.8141}}_{-\num{0.8063}}$ & ${}^{+\num{0.5146}}_{-\num{0.5116}}$ & ${}^{+\num{0.3200}}_{-\num{0.3179}}$ & ${}^{+\num{0.0803}}_{-\num{0.0807}}$ & ${}^{+\num{0.0181}}_{-\num{0.0165}}$\\
				Total SM & \num{3.0031}  & \num{1.8336}  & \num{1.4175}  & \num{1.1901}  & \num{0.7008}  & \num{0.1815}  & \num{0.0439} \\
				Stat. Error & \num{0.7324}  & \num{0.7322}  & \num{0.7133}  & \num{0.4505}  & \num{0.2585}  & \num{0.0746}  & \num{0.0014} \\
				Data & 5  & 2  & 2  & 2  & 0  & \num{0.2500} (1)  & \num{0.2500} (1) \\
				\makecell{RPV Wino $\lambda_{12k}\neq 0$ \\ $m(\tilde{\chi}_{1}^{\pm},\, \tilde{\chi}_{1}^{0}) = (900,\,400)$~GeV} & \num{0.0339}  & \num{0.1104}  & \num{0.1298}  & \num{0.1618}  & \num{0.3222}  & \num{0.5429}  & \num{0.7690} \\
			\hline
		\end{tabular}
	}	
\caption{Yields per $100\GeV$, and associated errors, 
	for each bin of the histogram Fig.~\ref{fig:SR0noZmeff} in SR0A and SR0B. 
	Values are rounded to two significant figures. 
	In the case where bins are wider than $100\GeV$ the actual number of data events in the bin is indicated in brackets. 
	The uppermost bin contains overflows.
}
\label{tb:aux_material_sr0ab_yields}		
}\end{table}

%Feb 2018
\begin{table}{\small
		\centering
		{\renewcommand{\arraystretch}{2}
			\begin{tabular}{llllll}
				\hline
				Component                                                &                                                             \multicolumn{4}{c}{Histogram Bin}                                                             &  \\
				                                                         & 6                                    & 7                                    & 8                                    & 9                                    & 10                                   \\ \hline
				min $\met ~[\GeV]$                                          & 50.0                                 & 60.0                                 & 70.0                                 & 80.0                                 & 90.0                                 \\
				max $\met ~[\GeV]$                                          & 60.0                                 & 70.0                                 & 80.0                                 & 90.0                                 & 100.0                                \\ \hline
				Other                                                    & \num{0.0000}                         & \num{0.0000}                         & \num{0.0000}                         & \num{0.0000}                         & \num{0.0000}                         \\
				VVV                                                      & \num{0.8843}                         & \num{0.5779}                         & \num{0.2660}                         & \num{0.2249}                         & \num{0.1925}                         \\
				Higgs                                                    & \num{0.1643}                         & \num{0.1313}                         & \num{0.1128}                         & \num{0.1146}                         & \num{0.0760}                         \\
				$t\bar{t}Z$                                              & \num{0.3131}                         & \num{0.3187}                         & \num{0.3125}                         & \num{0.3336}                         & \num{0.2858}                         \\
				ZZ                                                       & \num{14.8941}                        & \num{6.8594}                         & \num{3.3757}                         & \num{1.4505}                         & \num{0.6915}                         \\
				Reducible                                                & \num{0.0129}                         & \num{0.0000}                         & \num{1.0950}                         & \num{0.0000}                         & \num{0.0000}                         \\
				Stat. $\otimes$ Syst.                                    & ${}^{+\num{5.2839}}_{-\num{4.8350}}$ & ${}^{+\num{3.5964}}_{-\num{2.4810}}$ & ${}^{+\num{2.1088}}_{-\num{2.0324}}$ & ${}^{+\num{0.6921}}_{-\num{0.6844}}$ & ${}^{+\num{0.5977}}_{-\num{0.3819}}$ \\
				Total SM                                                 & \num{16.2688}                        & \num{7.8873}                         & \num{5.1621}                         & \num{2.1235}                         & \num{1.2459}                         \\
				Stat. Error                                              & \num{0.8069}                         & \num{0.5620}                         & \num{0.8467}                         & \num{0.1751}                         & \num{0.1136}                         \\
				Data                                                     & 17                                   & 12                                   & 5                                    & 2                                    & 1                                    \\
				\makecell{GGM ZZ \\ $m(\tilde{\chi}_{1}^{0}) = 400$~GeV} & \num{0.0515}                         & \num{0.0773}                         & \num{0.2315}                         & \num{0.0791}                         & \num{0.0291}                         \\ \hline
			\end{tabular}
		}
\caption{Yields per $10\GeV$, and associated errors, 
	for each bin of the histogram Fig.~\ref{fig:SR0Zmet} (part 1) in SR0C. 
	Values are rounded to two significant figures. 
}	
}\end{table}



%Feb 2018
\begin{table}{\small
		\centering
		{\renewcommand{\arraystretch}{2}
			\begin{tabular}{lllll}
				\hline
				Component                                                &                                         \multicolumn{3}{c}{Histogram Bin}                                          &  \\
				                                                         & 11                                   & 12                                   & 13                                   & 14                                   \\ \hline
				min $\met ~[\GeV]$                                          & 100.0                                & 150.0                                & 200.0                                & 250.0                                \\
				max $\met ~[\GeV]$                                          & 150.0                                & 200.0                                & 250.0                                & 260.0                                \\ \hline
				Other                                                    & \num{0.0000}                         & \num{0.1108}                         & \num{0.0000}                         & \num{0.2922}                         \\
				VVV                                                      & \num{0.0689}                         & \num{0.0237}                         & \num{0.0179}                         & \num{0.0925}                         \\
				Higgs                                                    & \num{0.0447}                         & \num{0.0082}                         & \num{0.0013}                         & \num{0.0109}                         \\
				$t\bar{t}Z$                                              & \num{0.2024}                         & \num{0.0748}                         & \num{0.0301}                         & \num{0.1132}                         \\
				ZZ                                                       & \num{0.1467}                         & \num{0.0091}                         & \num{0.0027}                         & \num{0.0112}                         \\
				Reducible                                                & \num{0.0624}                         & \num{0.0000}                         & \num{0.0000}                         & \num{0.0000}                         \\
				Stat. $\otimes$ Syst.                                    & ${}^{+\num{0.1325}}_{-\num{0.1270}}$ & ${}^{+\num{0.0257}}_{-\num{0.0242}}$ & ${}^{+\num{0.0151}}_{-\num{0.0108}}$ & ${}^{+\num{0.0499}}_{-\num{0.0484}}$ \\
				Total SM                                                 & \num{0.5251}                         & \num{0.2266}                         & \num{0.0520}                         & \num{0.5200}                         \\
				Stat. Error                                              & \num{0.0823}                         & \num{0.1110}                         & \num{0.0058}                         & \num{0.2933}                         \\
				Data                                                     & \num{1.2000} (6)                     & \num{0.2000} (1)                      & \num{0.6000} (3)                    & 0          \\
				\makecell{GGM ZZ \\ $m(\tilde{\chi}_{1}^{0}) = 400$~GeV} & \num{0.1573}                         & \num{0.1720}                         & \num{0.1719}                         & \num{2.0975}                         \\ \hline
			\end{tabular}
		}
\caption{Yields per $10\GeV$, and associated errors, 
	for each bin of the histogram Fig.~\ref{fig:SR0noZmeff} in SR0C (part 2) and SR0D. 
	Values are rounded to two significant figures. 
	In the case where bins are wider than $10\GeV$ the actual number of data events in the bin is indicated in brackets. 
	The uppermost bin contains overflows.
}
		\label{tb:aux_material_sr_D_yields}
}\end{table}


\begin{table}{\small
		\centering
		{\renewcommand{\arraystretch}{2}
			\begin{tabular}{lllll}
				\hline
				Component  &   \multicolumn{3}{c}{Histogram Bin}                                            &  \\
				& 8                                  & 9             & 10                                   & 11                                   \\
				min $\meff ~[\GeV]$   					 & 700.0      	 & 1100.0                               & 1500.0                               & 1900.0                               \\
				max $\meff ~[\GeV]$                      & 1100.0        & 1500.0                               & 1900.0                               & 2000.0                               \\ \hline
				Other                                                                                                              & \num{0.0345}                         & \num{0.0027}                         & \num{0.0046}                         & \num{0.0034}                         \\
				VVV                                                                                                                & \num{0.0345}                         & \num{0.0027}                         & \num{0.0046}                         & \num{0.0034}                         \\
				Higgs                                                                                                              & \num{0.0996}                         & \num{0.0154}                         & \num{0.0009}                         & \num{0.0001}                         \\
				$t\bar{t}Z$                                                                                                        & \num{0.0793}                         & \num{0.0159}                         & \num{0.0014}                         & \num{0.0034}                         \\
				ZZ                                                                                                                 & \num{0.0722}                         & \num{0.0157}                         & \num{0.0023}                         & \num{0.0030}                         \\
				Reducible                                                                                                          & \num{0.4413}                         & \num{0.1846}                         & \num{0.1125}                         & \num{0.1678}                         \\
				Stat. $\otimes$ Syst.                                                                                              & ${}^{+\num{0.1777}}_{-\num{0.1779}}$ & ${}^{+\num{0.0524}}_{-\num{0.0523}}$ & ${}^{+\num{0.0313}}_{-\num{0.0312}}$ & ${}^{+\num{0.1723}}_{-\num{0.1722}}$ \\
				Total SM                                                                                                           & \num{0.7553}                         & \num{0.2543}                         & \num{0.1245}                         & \num{0.1800}                         \\
				Stat. Error                                                                                                        & \num{0.2650}                         & \num{0.1481}                         & \num{0.1193}                         & \num{0.1153}                         \\
				Data                                 & \num{1.5000} (6)                     & \num{0.2500} (1)                     & \num{0.2500} (1)                     & 0                        \\
				\makecell{RPV Wino $\lambda_{i33}\neq 0$ \\ $m(\tilde{\chi}_{1}^{\pm},\,\tilde{\chi}_{1}^{0}) = (500,\, 200)$~GeV} & \num{4.6317}                         & \num{0.9203}                         & \num{0.2118}                         & \num{0.2757}                         \\ \hline
			\end{tabular}
		}
\label{tb:aux_material_sr1_yields}
\caption{Yields per $100\GeV$, and associated errors, 
	for each bin of the histogram Fig.~\ref{fig:SR1meff} in SR1. 
	Values are rounded to two significant figures. 
	In the case where bins are wider than $100\GeV$ the actual number of data events in the bin is indicated in brackets. 
	The uppermost bin contains overflows.
}	
}\end{table}

%Feb 2018
\begin{table}{\small
		\centering
		{\renewcommand{\arraystretch}{2}
			\begin{tabular}{llllll}
				\hline
				Component   &                                                             \multicolumn{4}{c}{Histogram Bin}                                                             &  \\
				& 7                                    & 8                                    & 9                                    & 10                                   & 11                                   \\ \hline
				min $\meff ~[\GeV]$                      & 600.0                                & 700.0                                & 1100.0                               & 1500.0        & 1900.0                               \\
				max $\meff ~[\GeV]$                      & 700.0                                & 1100.0                               & 1500.0                               & 1900.0        & 2000.0                               \\ \hline
				Other                                                                                                              & \num{0.0000}                         & \num{0.0209}                         & \num{0.0000}                         & \num{0.0000}                         & \num{0.0000}                         \\
				VVV                                                                                                                & \num{0.0514}                         & \num{0.0120}                         & \num{0.0031}                         & \num{0.0014}                         & \num{0.0022}                         \\
				Higgs                                                                                                              & \num{0.1106}                         & \num{0.0457}                         & \num{0.0050}                         & \num{0.0002}                         & \num{0.0025}                         \\
				$t\bar{t}Z$                                                                                                        & \num{0.1143}                         & \num{0.0256}                         & \num{0.0048}                         & \num{0.0000}                         & \num{0.0000}                         \\
				ZZ                                                                                                                 & \num{0.1298}                         & \num{0.0399}                         & \num{0.0073}                         & \num{0.0015}                         & \num{0.0027}                         \\
				Reducible                                                                                                          & \num{0.0000}                         & \num{0.2157}                         & \num{0.0315}                         & \num{0.0033}                         & \num{0.0000}                         \\
				Stat. $\otimes$ Syst.                                                                                              & ${}^{+\num{0.3957}}_{-\num{0.3945}}$ & ${}^{+\num{0.0932}}_{-\num{0.0923}}$ & ${}^{+\num{0.0176}}_{-\num{0.0178}}$ & ${}^{+\num{0.0053}}_{-\num{0.0053}}$ & ${}^{+\num{0.0504}}_{-\num{0.0505}}$ \\
				Total SM                                                                                                           & \num{0.4062}                         & \num{0.3597}                         & \num{0.0517}                         & \num{0.0064}                         & \num{0.0074}                         \\
				Stat. Error                                                                                                        & \num{0.3105}                         & \num{0.1338}                         & \num{0.0500}                         & \num{0.0189}                         & \num{0.0354}                         \\
				Data                                 & 0                       & \num{0.2500} (1)                         & \num{0.2500}  (1)                       & 0                       & 0                      \\
				\makecell{RPV Wino $\lambda_{i33}\neq 0$ \\ $m(\tilde{\chi}_{1}^{\pm},\,\tilde{\chi}_{1}^{0}) = (500,\, 200)$~GeV} & \num{2.7939}                         & \num{1.9461}                         & \num{0.4911}                         & \num{0.1549}                         & \num{0.3870}                         \\ \hline
			\end{tabular}
		}
		\caption{Yields per $100\GeV$, and associated errors, 
			for each bin of the histogram Fig.~\ref{fig:SR2meff} in SR2. 
			Values are rounded to two significant figures. 
			In the case where bins are wider than $100\GeV$ the actual number of data events in the bin is indicated in brackets. 
			The uppermost bin contains overflows.
	}
		\label{tb:aux_material_sr2_yields}
}\end{table}





\FloatBarrier

%%%%%%%%%%%% Model Acceptances and Efficiencies

\begin{table}[h] { \small % Aux Tab 7
\begin{center}
\begin{tabular}{l l  |  c c c }
\toprule
\multicolumn{2}{c}{Masses ~$[\GeV]$} & \multicolumn{3}{c}{Efficiency} \\ 
$m_{\mathrm NLSP}$ & $m_{LSP}$ & $A$(particle) & $\epsilon$(reco) & $\epsilon$(reco) $\times$ $A$(particle) \\ 
\toprule
 1200 & 10 &   0.35 & 0.43  & 0.15 \\
 1200 & 50 &   0.70 & 0.56  & 0.40 \\
 1200 & 200 &  0.63 & 0.81  & 0.51 \\
 1200 & 600 &  0.75 & 0.86  & 0.64 \\
 1200 & 800 &  0.74 & 0.88  & 0.65 \\
 1200 & 1000 & 0.73 & 0.87  & 0.64 \\
 1200 & 1190 & 0.77 & 0.77  & 0.60 \\
%
\bottomrule
\end{tabular}
\end{center}
\caption{ Acceptance ($A$) at particle level in simulation and selection efficiency ($\epsilon$) at reconstruction level 
for the Wino  $\chinoonep\chinoonem$ $\LLE 12k$ model fulfilling the selection criteria of SR0A.
The implementation of ``simple'' cut selection at truth level uses the {\textsc{SimpleAnalysis}} framework 
and the code can be found at this link \href{https://gitlab.cern.ch/atlas-phys-susy-wg/SimpleAnalysis/blob/master/Root/FourLepton2016.cxx}{FourLepton2016}.
} 
\label{tb:sr_and_model} }
\end{table}
    
    

    
\begin{table}[h] { \small % Aux Tab 8
\begin{center}
\begin{tabular}{l l  |  c c c }
\toprule
\multicolumn{2}{c}{Masses ~$[\GeV]$} & \multicolumn{3}{c}{Efficiency} \\ 
$m_{\mathrm NLSP}$ & $m_{LSP}$ & $A$(particle) & $\epsilon$(reco) & $\epsilon$(reco) $\times$ $A$(particle) \\ 
\toprule
1200 & 10 &  0.31 & 0.39  & 0.12 \\
1200 & 50 &  0.65 & 0.54  & 0.35 \\
1200 & 200 &   0.57 & 0.76  & 0.44 \\
1200 & 600 &   0.69 & 0.83  & 0.57 \\
1200 & 1190 &  0.77 & 0.78  & 0.60 \\
\bottomrule
\end{tabular}
\end{center}
\caption{  Acceptance ($A$) at particle level in simulation and selection efficiency ($\epsilon$) at reconstruction level 
for the Wino $\chinoonepm\ninotwo\; Z$  $\LLE 12k$ model passing the selection criteria of SR0A.
The implementation of ``simple'' cut selection at truth level uses the {\textsc{SimpleAnalysis}} framework 
and the code can be found at this link \href{https://gitlab.cern.ch/atlas-phys-susy-wg/SimpleAnalysis/blob/master/Root/FourLepton2016.cxx}{FourLepton2016}.
} 
\label{tb:eff_acc_sr0b_c1n2z} }
\end{table}




\begin{table}[h] { \small % Aux Tab 9
\begin{center}
\begin{tabular}{l l  |  c c c }
	\toprule
	\multicolumn{2}{c}{Masses ~$[\GeV]$} &                    \multicolumn{3}{c}{Efficiency}                    \\
	$m_{\mathrm NLSP}$ & $m_{LSP}$   & $A$(particle) & $\epsilon$(reco) & $\epsilon$(reco) $\times$ $A$(particle) \\ \toprule
	1200   			   & 10          & 0.33      & 0.41            & 0.13                                \\
	1200               & 50          & 0.68      & 0.53            & 0.36                                \\
	1200               & 200         & 0.60      & 0.81            & 0.49                                \\
	1200               & 600         & 0.70      & 0.81            & 0.57                                \\
	1200               & 1070        & 0.69      & 0.89            & 0.61                                \\ \bottomrule
\end{tabular}
\end{center}
\caption{  Acceptance ($A$) at particle level in simulation and selection efficiency ($\epsilon$) at reconstruction level 
for the Wino $\chinoonepm\ninotwo\; h$  $\LLE 12k$ model passing the selection criteria of SR0A.
The implementation of ``simple'' cut selection at truth level uses the {\textsc{SimpleAnalysis}} framework 
and the code can be found at this link \href{https://gitlab.cern.ch/atlas-phys-susy-wg/SimpleAnalysis/blob/master/Root/FourLepton2016.cxx}{FourLepton2016}.
} 
\label{tb:eff_acc_sr0b_c1n2h} }
\end{table}



\begin{table}[h] { \small % Aux Tab 10
\begin{center}
\begin{tabular}{l l  |  c c c }
	\toprule
	\multicolumn{2}{c}{Masses ~$[\GeV]$} &                    \multicolumn{3}{c}{Efficiency}                    \\
	$m_{\mathrm NLSP}$ & $m_{LSP}$   & $A$(particle) & $\epsilon$(reco) & $\epsilon$(reco) $\times$ $A$(particle) \\ \toprule
        1200  		   & 10          & 0.43      & 0.51            & 0.22                                \\
	1200               & 50          & 0.79      & 0.62            & 0.48                                \\
	1200               & 200         & 0.71      & 0.85            & 0.60                                \\
	1200               & 600         & 0.87      & 0.87            & 0.76                                \\
	1200               & 1000        & 0.88      & 0.88            & 0.77                                \\
	1200               & 1190        & 0.80      & 0.80            & 0.64                                \\ \bottomrule
\end{tabular}
\end{center}
\caption{ Acceptance ($A$) at particle level in simulation and selection efficiency ($\epsilon$) at reconstruction level 
for the slepton/sneutrino $\LLE 12k$ model passing the selection criteria of SR0A.
The implementation of ``simple'' cut selection at truth level uses the {\textsc{SimpleAnalysis}} framework 
and the code can be found at this link \href{https://gitlab.cern.ch/atlas-phys-susy-wg/SimpleAnalysis/blob/master/Root/FourLepton2016.cxx}{FourLepton2016}.
} 
\label{tb:eff_acc_sr0b_gluino} }
\end{table}




\begin{table}[h] { \small % Aux Tab 11
\begin{center}
\begin{tabular}{l l  |  c c c }
	\toprule
	\multicolumn{2}{c}{Masses ~$[\GeV]$} &                    \multicolumn{3}{c}{Efficiency}                    \\
	$m_{\mathrm NLSP}$ & $m_{LSP}$   & $A$(particle) & $\epsilon$(reco) & $\epsilon$(reco) $\times$ $A$(particle) \\ \toprule
	1500   		   & 50          & 0.54      & 0.42            & 0.23                                \\
	1500               & 100         & 0.47      & 0.56            & 0.26                                \\
	1500               & 500         & 0.60      & 0.77            & 0.46                                \\
	1500               & 1100        & 0.62      & 0.83            & 0.51                                \\
	1500               & 1490        & 0.75      & 0.77            & 0.57                                \\ \bottomrule
\end{tabular}
\end{center}
\caption{ Acceptance ($A$) at particle level in simulation and selection efficiency ($\epsilon$) at reconstruction level for the $\gluino\gluino$ $\LLE 12k$ model passing the selection criteria of SR0A.
The implementation of ``simple'' cut selection at truth level uses the {\textsc{SimpleAnalysis}} framework 
and the code can be found at this link \href{https://gitlab.cern.ch/atlas-phys-susy-wg/SimpleAnalysis/blob/master/Root/FourLepton2016.cxx}{FourLepton2016}.
} 
\label{tb:eff_acc_sr0b_gluino} }
\end{table}

\begin{table}[h] { \small % Aux Tab 12
\begin{center}
\begin{tabular}{l l  |  c c c }
	\toprule
	\multicolumn{2}{c}{Masses ~$[\GeV]$} &                    \multicolumn{3}{c}{Efficiency}                    \\
	$m_{\mathrm NLSP}$ & $m_{LSP}$   & $A$(particle) & $\epsilon$(reco) & $\epsilon$(reco) $\times$ $A$(particle) \\ \toprule
        1200		   & 10          & 0.33      & 0.43            & 0.14                                \\
	1200               & 50          & 0.68      & 0.55            & 0.38                                \\
	1200               & 200         & 0.61      & 0.80            & 0.49                                \\
	1200               & 600         & 0.74      & 0.86            & 0.63                                \\
	1200               & 800         & 0.73      & 0.88            & 0.64                                \\
	1200               & 1000        & 0.72      & 0.87            & 0.63                                \\
	1200               & 1190        & 0.76      & 0.77            & 0.59                                \\ \bottomrule
\end{tabular}
\end{center}
\caption{ Acceptance ($A$) at particle level in simulation and selection efficiency ($\epsilon$) at reconstruction level 
for the Wino  $\chinoonep\chinoonem$ $\LLE 12k$ model passing the selection criteria of SR0B.
The implementation of ``simple'' cut selection at truth level uses the {\textsc{SimpleAnalysis}} framework 
and the code can be found at this link \href{https://gitlab.cern.ch/atlas-phys-susy-wg/SimpleAnalysis/blob/master/Root/FourLepton2016.cxx}{FourLepton2016}.
} 
\label{tb:sr_and_model} }
\end{table}
    
    
\begin{table}[h] { \small % Aux Tab 13
\begin{center}
\begin{tabular}{l l  |  c c c }
	\toprule
	\multicolumn{2}{c}{Masses ~$[\GeV]$} &                    \multicolumn{3}{c}{Efficiency}                    \\
	$m_{\mathrm NLSP}$ & $m_{LSP}$   & $A$(particle) & $\epsilon$(reco) & $\epsilon$(reco) $\times$ $A$(particle) \\ \toprule
	1200   		   & 10          & 0.30      & 0.39            & 0.12                                \\
	1200               & 50          & 0.62      & 0.54            & 0.33                                \\
	1200               & 200         & 0.55      & 0.76            & 0.42                                \\
	1200               & 600         & 0.67      & 0.82            & 0.55                                \\
	1200               & 1190        & 0.76      & 0.78            & 0.59                                \\ \bottomrule
\end{tabular}
\end{center}
\caption{Acceptance ($A$) at particle level in simulation and selection efficiency ($\epsilon$) at reconstruction level 
for the Wino $\chinoonepm\ninotwo\; Z$  $\LLE 12k$ model passing the selection criteria of SR0B.
The implementation of ``simple'' cut selection at truth level uses the {\textsc{SimpleAnalysis}} framework 
and the code can be found at this link \href{https://gitlab.cern.ch/atlas-phys-susy-wg/SimpleAnalysis/blob/master/Root/FourLepton2016.cxx}{FourLepton2016}.
} 
\label{tb:eff_acc_sr0b_c1n2z} }
\end{table}




\begin{table}[h] { \small % Aux Tab 14
\begin{center}
\begin{tabular}{l l  |  c c c }
	\toprule
	\multicolumn{2}{c}{Masses ~$[\GeV]$} &                    \multicolumn{3}{c}{Efficiency}                    \\
	$m_{\mathrm NLSP}$ & $m_{LSP}$   & $A$(particle) & $\epsilon$(reco) & $\epsilon$(reco) $\times$ $A$(particle) \\ \toprule
	1200		   & 10          & 0.32      & 0.41            & 0.13                                \\
	1200               & 50          & 0.67      & 0.53            & 0.35                                \\
	1200               & 200         & 0.58      & 0.81            & 0.47                                \\
	1200               & 600         & 0.69      & 0.81            & 0.56                                \\
	1200               & 1070        & 0.67      & 0.89            & 0.60                                \\ \bottomrule
\end{tabular}
\end{center}
\caption{ Acceptance ($A$) at particle level in simulation and selection efficiency ($\epsilon$) at reconstruction level 
for the Wino $\chinoonepm\ninotwo\; h$  $\LLE 12k$ model passing the selection criteria of SR0B.
The implementation of ``simple'' cut selection at truth level uses the {\textsc{SimpleAnalysis}} framework 
and the code can be found at this link \href{https://gitlab.cern.ch/atlas-phys-susy-wg/SimpleAnalysis/blob/master/Root/FourLepton2016.cxx}{FourLepton2016}.
} 
\label{tb:eff_acc_sr0b_c1n2h} }
\end{table}




\begin{table}[h] { \small % Aux Tab 15
\begin{center}
\begin{tabular}{l l  |  c c c }
	\toprule
	\multicolumn{2}{c}{Masses ~$[\GeV]$} &                    \multicolumn{3}{c}{Efficiency}                    \\
	$m_{\mathrm NLSP}$ & $m_{LSP}$   & $A$(particle) & $\epsilon$(reco) & $\epsilon$(reco) $\times$ $A$(particle) \\ \toprule
        1200		   & 10          & 0.41      & 0.52            & 0.21                                \\
	1200               & 50          & 0.74      & 0.62            & 0.46                                \\
	1200               & 200         & 0.67      & 0.86            & 0.58                                \\
	1200               & 600         & 0.83      & 0.88            & 0.73                                \\
	1200               & 1000        & 0.87      & 0.87            & 0.76                                \\
	1200               & 1190        & 0.79      & 0.80            & 0.63                                \\
	\bottomrule
\end{tabular}
\end{center}
\caption{Acceptance ($A$) at particle level in simulation and selection efficiency ($\epsilon$) at reconstruction level 
for the slepton/sneutrino $\LLE 12k$ model passing the selection criteria of SR0B.
The implementation of ``simple'' cut selection at truth level uses the {\textsc{SimpleAnalysis}} framework 
and the code can be found at this link \href{https://gitlab.cern.ch/atlas-phys-susy-wg/SimpleAnalysis/blob/master/Root/FourLepton2016.cxx}{FourLepton2016}.
} 
\label{tb:eff_acc_sr0b_gluino} }
\end{table}





\begin{table}[h] { \small % Aux Tab 16
\begin{center}
\begin{tabular}{l l  |  c c c }
	\toprule
	\multicolumn{2}{c}{Masses ~$[\GeV]$} &                    \multicolumn{3}{c}{Efficiency}                    \\
	$m_{\mathrm NLSP}$ & $m_{LSP}$   & $A$(particle) & $\epsilon$(reco) & $\epsilon$(reco) $\times$ $A$(particle) \\ \toprule
        1500		   & 10          & 0.26      & 0.25            & 0.07                                \\
	1500               & 50          & 0.54      & 0.42            & 0.23                                \\
	1500               & 100         & 0.47      & 0.56            & 0.26                                \\
	1500               & 500         & 0.60      & 0.77            & 0.46                                \\
	1500               & 1100        & 0.62      & 0.83            & 0.51                                \\
	1500               & 1490        & 0.75      & 0.77            & 0.57                                \\ \bottomrule
\end{tabular}
\end{center}
\caption{ Acceptance ($A$) at particle level in simulation and selection efficiency ($\epsilon$) at reconstruction level 
for the $\gluino\gluino$ $\LLE 12k$ model passing the selection criteria of SR0B.
The implementation of ``simple'' cut selection at truth level uses the {\textsc{SimpleAnalysis}} framework 
and the code can be found at this link \href{https://gitlab.cern.ch/atlas-phys-susy-wg/SimpleAnalysis/blob/master/Root/FourLepton2016.cxx}{FourLepton2016}.
} 
\label{tb:eff_acc_sr0b_gluino} }
\end{table}

\begin{table}[h] { \small % Aux Tab 17
\begin{center}
\begin{tabular}{l l  |  c c c }
\toprule
Mass ~$[\GeV]$ & $\mathrm{BR}$ & \multicolumn{3}{c}{Efficiency} \\ 
$m_{\mathrm NLSP}$ & $\ninoone \ra Z \gravino$ & $A$(particle) & $\epsilon$(reco) & $\epsilon$(reco) $\times$ $A$(particle) \\ 
\toprule
400 & 100\% &  0.246 & 0.0069 & 0.002 \\ 
\hline
400 & 50\%   & 0.007 & 0.0547  &  0.0004\\
\bottomrule
\end{tabular}
\end{center}
\caption{ Acceptance ($A$) at particle level in simulation and selection efficiency ($\epsilon$) at reconstruction level 
for the GGM higgsino models with $\mathrm{BR}(\ninoone \ra Z \gravino)=100\%$ (top) and $\mathrm{BR}(\ninoone \ra Z \gravino)=50\%$ (bottom) fulfilling the selection criteria of SR0C.
The implementation of ``simple'' cut selection at truth level uses the {\textsc{SimpleAnalysis}} framework 
and the code can be found at this link \href{https://gitlab.cern.ch/atlas-phys-susy-wg/SimpleAnalysis/blob/master/Root/FourLepton2016.cxx}{FourLepton2016}.
} 
\label{tb:acc_sr0d_ggm} }
\end{table}

\begin{table}[h] { \small % Aux Tab 18
\begin{center}
\begin{tabular}{l l  |  c c c }
\toprule
Mass ~$[\GeV]$ & $\mathrm{BR}$ & \multicolumn{3}{c}{Efficiency} \\ 
$m_{\mathrm NLSP}$ & $\ninoone \ra Z \gravino$ & $A$(particle) & $\epsilon$(reco) & $\epsilon$(reco) $\times$ $A$(particle) \\ 
\toprule
400 & 100\% & 0.222 & 0.0068 & 0.002 \\ 
\hline
400 & 50\%  & 0.006 & 0.0542 & 0.0003 \\ 
\bottomrule
\end{tabular}
\end{center}
\caption{ Acceptance ($A$) at particle level in simulation and selection efficiency ($\epsilon$) at reconstruction level 
for the GGM higgsino models with $\mathrm{BR}(\ninoone \ra Z \gravino)=100\%$ (top) and $\mathrm{BR}(\ninoone \ra Z \gravino)=50\%$ (bottom) fulfilling the selection criteria of SR0D.
The implementation of ``simple'' cut selection at truth level uses the {\textsc{SimpleAnalysis}} framework 
and the code can be found at this link \href{https://gitlab.cern.ch/atlas-phys-susy-wg/SimpleAnalysis/blob/master/Root/FourLepton2016.cxx}{FourLepton2016}.
} 
\label{tb:acc_sr0d_ggm} }
\end{table}

\begin{table}[h] { \small % Aux Tab 19
\begin{center}
\begin{tabular}{l l  |  c c c }
	\toprule
	\multicolumn{2}{c}{Masses ~$[\GeV]$} &                    \multicolumn{3}{c}{Efficiency}                    \\
	$m_{\mathrm NLSP}$ & $m_{LSP}$   & $A$(particle) & $\epsilon$(reco) & $\epsilon$(reco) $\times$ $A$(particle) \\ \toprule
        800                & 10          & 0.02      & 0.05            & 0.001                                \\
	800                & 500         & 0.06      & 0.20            & 0.01                                \\
	800                & 100         & 0.09      & 0.37            & 0.03                                \\
	800                & 200         & 0.12      & 0.52            & 0.06                                \\
	800                & 300         & 0.13      & 0.50            & 0.07                                \\
	800                & 400         & 0.13      & 0.59            & 0.08                                \\
	800                & 500         & 0.13      & 0.55            & 0.07                                \\
	800                & 600         & 0.14      & 0.55            & 0.08                                \\
	800                & 700         & 0.13      & 0.54            & 0.07                                \\
	800                & 790         & 0.11      & 0.46            & 0.05                                \\ \bottomrule
\end{tabular}
\end{center}
\caption{  Acceptance ($A$) at particle level in simulation and selection efficiency ($\epsilon$) at reconstruction level 
for the Wino  $\chinoonep\chinoonem$ $\LLE i33$ model passing the selection criteria of SR1.
The implementation of ``simple'' cut selection at truth level uses the {\textsc{SimpleAnalysis}} framework 
and the code can be found at this link \href{https://gitlab.cern.ch/atlas-phys-susy-wg/SimpleAnalysis/blob/master/Root/FourLepton2016.cxx}{FourLepton2016}.
} 
\label{tb:sr_and_model} }
\end{table}
    
    

    
    
\begin{table}[h] { \small % Aux Tab 20
\begin{center}
\begin{tabular}{l l  |  c c c }
	\toprule
	\multicolumn{2}{c}{Masses ~$[\GeV]$} &                    \multicolumn{3}{c}{Efficiency}                    \\
	$m_{\mathrm NLSP}$ & $m_{LSP}$   & $A$(particle) & $\epsilon$(reco) & $\epsilon$(reco) $\times$ $A$(particle) \\ \toprule
	800		   & 100         & 0.08      & 0.31            & 0.03                                \\
	800                & 400         & 0.11      & 0.46            & 0.05                                \\
	800                & 790         & 0.10      & 0.41            & 0.04                                \\ \bottomrule
\end{tabular}
\end{center}
\caption{  Acceptance ($A$) at particle level in simulation and selection efficiency ($\epsilon$) at reconstruction level 
for the Wino $\chinoonepm\ninotwo\; Z$  $\LLE i33$ model passing the selection criteria of SR1.
The implementation of ``simple'' cut selection at truth level uses the {\textsc{SimpleAnalysis}} framework 
and the code can be found at this link \href{https://gitlab.cern.ch/atlas-phys-susy-wg/SimpleAnalysis/blob/master/Root/FourLepton2016.cxx}{FourLepton2016}.
} 
\label{tb:eff_acc_sr0b_c1n2z} }
\end{table}




\begin{table}[h] { \small % Aux Tab 21
\begin{center}
\begin{tabular}{l l  |  c c c }
\toprule
\multicolumn{2}{c}{Masses ~$[\GeV]$} & \multicolumn{3}{c}{Efficiency} \\ 
$m_{\mathrm NLSP}$ & $m_{LSP}$ & $A$(particle) & $\epsilon$(reco) & $\epsilon$(reco) $\times$ $A$(particle) \\ 
\toprule
 800 & 100 &  0.09 & 0.38  & 0.03 \\
 800 & 400 &  0.12 & 0.48  & 0.06 \\
 800 & 670 &  0.12 & 0.49  & 0.06 \\
\bottomrule
\end{tabular}
\end{center}
\caption{  Acceptance ($A$) at particle level in simulation and selection efficiency ($\epsilon$) at reconstruction level 
for the Wino $\chinoonepm\ninotwo\; h$  $\LLE i33$ model passing the selection criteria of SR1.
The implementation of ``simple'' cut selection at truth level uses the {\textsc{SimpleAnalysis}} framework 
and the code can be found at this link \href{https://gitlab.cern.ch/atlas-phys-susy-wg/SimpleAnalysis/blob/master/Root/FourLepton2016.cxx}{FourLepton2016}.
} 
\label{tb:eff_acc_sr0b_c1n2h} }
\end{table}




\begin{table}[h] { \small % Aux Tab 22
\begin{center}
\begin{tabular}{l l  |  c c c }
	\toprule
	\multicolumn{2}{c}{Masses ~$[\GeV]$} &                    \multicolumn{3}{c}{Efficiency}                    \\
	$m_{\mathrm NLSP}$ & $m_{LSP}$   & $A$(particle) & $\epsilon$(reco) & $\epsilon$(reco) $\times$ $A$(particle) \\ \toprule
	800                & 100         & 0.12      & 0.55            & 0.07                                \\
	800                & 300         & 0.17      & 0.79            & 0.13                                \\
	800                & 700         & 0.18      & 0.77            & 0.14                                \\
	800                & 790         & 0.15      & 0.58            & 0.09
\end{tabular}
\end{center}
\caption{  Acceptance ($A$) at particle level in simulation and selection efficiency ($\epsilon$) at reconstruction level 
for the slepton/sneutrino $\LLE i33$ model passing the selection criteria of SR1.
The implementation of ``simple'' cut selection at truth level uses the {\textsc{SimpleAnalysis}} framework 
and the code can be found at this link \href{https://gitlab.cern.ch/atlas-phys-susy-wg/SimpleAnalysis/blob/master/Root/FourLepton2016.cxx}{FourLepton2016}.
} 
\label{tb:eff_acc_sr0b_gluino} }
\end{table}





\begin{table}[h] { \small % Aux Tab 23
\begin{center}
\begin{tabular}{l l  |  c c c }
	\toprule
	\multicolumn{2}{c}{Masses ~$[\GeV]$} &                    \multicolumn{3}{c}{Efficiency}                    \\
	$m_{\mathrm NLSP}$  & $m_{LSP}$  & $A$(particle) & $\epsilon$(reco) & $\epsilon$(reco) $\times$ $A$(particle) \\ \toprule
        1000		    & 10         & 0.001      & 0.015            & 0.000                                \\
	1000                & 50         & 0.03      & 0.08            & 0.002                                \\
	1000                & 100        & 0.05      & 0.17            & 0.008                                \\
	1000                & 500        & 0.08      & 0.29            & 0.02                                \\
	1000                & 990        & 0.09      & 0.36            & 0.03                                \\ \bottomrule\bottomrule
\end{tabular}
\end{center}
\caption{ Acceptance ($A$) at particle level in simulation and selection efficiency ($\epsilon$) at reconstruction level 
for the $\gluino\gluino$ $\LLE i33$ model passing the selection criteria of SR1.
The implementation of ``simple'' cut selection at truth level uses the {\textsc{SimpleAnalysis}} framework 
and the code can be found at this link \href{https://gitlab.cern.ch/atlas-phys-susy-wg/SimpleAnalysis/blob/master/Root/FourLepton2016.cxx}{FourLepton2016}.
} 
\label{tb:eff_acc_sr0b_gluino} }
\end{table}

\begin{table}[h] { \small % Aux Tab 24
\begin{center}
\begin{tabular}{l l  |  c c c }
\toprule
\multicolumn{2}{c}{Masses ~$[\GeV]$} & \multicolumn{3}{c}{Efficiency} \\ 
$m_{\mathrm NLSP}$ & $m_{LSP}$ & $A$(particle) & $\epsilon$(reco) & $\epsilon$(reco) $\times$ $A$(particle) \\ 
\toprule
 800 & 10  &  0.02 & 0.003  & 0.000 \\
 800 & 50  &  0.05 & 0.05  & 0.002 \\
 800 & 100 &  0.08 & 0.25  & 0.02 \\
 800 & 200 &  0.10 & 0.45  & 0.04 \\
 800 & 300 &  0.10 & 0.48  & 0.05 \\
 800 & 400 &  0.11 & 0.55  & 0.06 \\
 800 & 500 &  0.11 & 0.51  & 0.06 \\
 800 & 600 &  0.10 & 0.53  & 0.05 \\
 800 & 700 &  0.11 & 0.46  & 0.05 \\
 800 & 790 &  0.11 & 0.36  & 0.04 \\
\bottomrule
\end{tabular}
\end{center}
\caption{ Acceptance ($A$) at particle level in simulation and selection efficiency ($\epsilon$) at reconstruction level
for the Wino  $\chinoonep\chinoonem$ $\LLE i33$ model passing the selection criteria of SR2.
The implementation of ``simple'' cut selection at truth level uses the {\textsc{SimpleAnalysis}} framework 
and the code can be found at this link \href{https://gitlab.cern.ch/atlas-phys-susy-wg/SimpleAnalysis/blob/master/Root/FourLepton2016.cxx}{FourLepton2016}.
} 
\label{tb:sr_and_model} }
\end{table}
    
    

    
\begin{table}[h] { \small % Aux Tab 25
\begin{center}
\begin{tabular}{l l  |  c c c }
\toprule
\multicolumn{2}{c}{Masses ~$[\GeV]$} & \multicolumn{3}{c}{Efficiency} \\ 
$m_{\mathrm NLSP}$ & $m_{LSP}$ & $A$(particle) & $\epsilon$(reco) & $\epsilon$(reco) $\times$ $A$(particle) \\ 
\toprule
 800 & 100 &   0.07 & 0.20  & 0.01 \\
 800 & 400 &   0.11 & 0.38  & 0.04 \\
 800 & 790 &   0.12 & 0.35  & 0.04 \\
\bottomrule
\end{tabular}
\end{center}
\caption{ Acceptance ($A$) at particle level in simulation and selection efficiency ($\epsilon$) at reconstruction level
for the Wino $\chinoonepm\ninotwo\; Z$  $\LLE i33$ model passing the selection criteria of SR2.
The implementation of ``simple'' cut selection at truth level uses the {\textsc{SimpleAnalysis}} framework 
and the code can be found at this link \href{https://gitlab.cern.ch/atlas-phys-susy-wg/SimpleAnalysis/blob/master/Root/FourLepton2016.cxx}{FourLepton2016}.
} 
\label{tb:eff_acc_sr0b_c1n2z} }
\end{table}





\begin{table}[h] { \small % Aux Tab 26
\begin{center}
\begin{tabular}{l l  |  c c c }
\toprule
\multicolumn{2}{c}{Masses ~$[\GeV]$} & \multicolumn{3}{c}{Efficiency} \\ 
$m_{\mathrm NLSP}$ & $m_{LSP}$ & $A$(particle) & $\epsilon$(reco) & $\epsilon$(reco) $\times$ $A$(particle) \\ 
\toprule
 800 & 100 &  0.07 & 0.26  & 0.02 \\
 800 & 400 &  0.12 & 0.43  & 0.05 \\
 800 & 670 &  0.11 & 0.34  & 0.04 \\
\bottomrule
\end{tabular}
\end{center}
\caption{  Acceptance ($A$) at particle level in simulation and selection efficiency ($\epsilon$) at reconstruction level
for the Wino $\chinoonepm\ninotwo\; h$  $\LLE i33$ model passing the selection criteria of SR2.
The implementation of ``simple'' cut selection at truth level uses the {\textsc{SimpleAnalysis}} framework 
and the code can be found at this link \href{https://gitlab.cern.ch/atlas-phys-susy-wg/SimpleAnalysis/blob/master/Root/FourLepton2016.cxx}{FourLepton2016}.
} 
\label{tb:eff_acc_sr0b_c1n2h} }
\end{table}




\begin{table}[h] { \small % Aux Tab 27
\begin{center}
\begin{tabular}{l l  |  c c c }
\toprule
\multicolumn{2}{c}{Masses ~$[\GeV]$} & \multicolumn{3}{c}{Efficiency} \\ 
$m_{\mathrm NLSP}$ & $m_{LSP}$ & $A$(particle) & $\epsilon$(reco) & $\epsilon$(reco) $\times$ $A$(particle) \\ 
\toprule
 800 & 100 &   0.07 & 0.35  & 0.03 \\
 800 & 300 &   0.09 & 0.85  & 0.07 \\
 800 & 700 &   0.10 & 0.84  & 0.08 \\
 800 & 790 &   0.10 & 0.56  & 0.05 \\
%
\bottomrule
\end{tabular}
\end{center}
\caption{ Acceptance ($A$) at particle level in simulation and selection efficiency ($\epsilon$) at reconstruction level
for the slepton/sneutrino $\LLE i33$ model passing the selection criteria of SR2.
The implementation of ``simple'' cut selection at truth level uses the {\textsc{SimpleAnalysis}} framework 
and the code can be found at this link \href{https://gitlab.cern.ch/atlas-phys-susy-wg/SimpleAnalysis/blob/master/Root/FourLepton2016.cxx}{FourLepton2016}.
} 
\label{tb:eff_acc_sr0b_gluino} }
\end{table}





\begin{table}[h] { \small % Aux Tab 28
\begin{center}
\begin{tabular}{l l  |  c c c }
\toprule
\multicolumn{2}{c}{Masses ~$[\GeV]$} & \multicolumn{3}{c}{Efficiency} \\ 
$m_{\mathrm NLSP}$ & $m_{LSP}$ & $A$(particle) & $\epsilon$(reco) & $\epsilon$(reco) $\times$ $A$(particle) \\ 
\toprule
 1000 & 10 &  0.005 & 0.000  & 0.000 \\
 1000 & 50 &  0.03 & 0.02  & 0.001 \\
 1000 & 100 & 0.06 & 0.09  & 0.005 \\
 1000 & 500 & 0.12 & 0.20  & 0.02 \\
 1000 & 990 & 0.14 & 0.26  & 0.04 \\
%
\bottomrule
\end{tabular}
\end{center}
\caption{Acceptance ($A$) at particle level in simulation and selection efficiency ($\epsilon$) at reconstruction level
for the $\gluino\gluino$ $\LLE i33$ model passing the selection criteria of SR2.
The implementation of ``simple'' cut selection at truth level uses the {\textsc{SimpleAnalysis}} framework 
and the code can be found at this link \href{https://gitlab.cern.ch/atlas-phys-susy-wg/SimpleAnalysis/blob/master/Root/FourLepton2016.cxx}{FourLepton2016}.
} 
\label{tb:eff_acc_sr0b_gluino} }
\end{table}

\FloatBarrier 

% \subsection{Cutflows} 
%%% wino, gluino, slepton %%%
\begin{table}[h]{\tiny \centering
\begin{tabular}{ lcc | c ccc ccc ccc | cc}
\toprule
%
Model 
& \rotatebox[origin=c]{90}{$m_\mathrm{NLSP}$ ~$[\GeV]$}
& \rotatebox[origin=c]{90}{$m_\mathrm{LSP}$ ~$[\GeV]$}
%
& \rotatebox[origin=c]{90}{Initial} 
%
& \rotatebox[origin=c]{90}{Trigger} 
& \rotatebox[origin=c]{90}{Event Cleaning} 
& \rotatebox[origin=c]{90}{$N_{e/\mu}  \geq 1$} 
& \rotatebox[origin=c]{90}{$N_{e/\mu} \geq 2$} 
& \rotatebox[origin=c]{90}{ $N_{e/\mu} \geq 3$ } 
& \rotatebox[origin=c]{90}{ $N_{e/\mu} \geq 4$ } 
& \rotatebox[origin=c]{90}{ Z veto} 
& \rotatebox[origin=c]{90}{$m_{\text{eff}} > 600$~GeV  (SR0A)}
& \rotatebox[origin=c]{90}{ $m_{\text{eff}} > 1100$~GeV (SR0B)} 
& \rotatebox[origin=c]{90}{Efficiency SR0A}
& \rotatebox[origin=c]{90}{Efficiency SR0B} 
\\
\hline
wino $\chinoonep\chinoonem$ 	& 1200  & 600	& 7.08  & 6.77  & 6.63  & 6.63  & 6.61  & 6.29  & 4.84 & 4.56 & 4.56 & 4.47 & 0.64 & 0.63 \\%A03
wino $\chinoonepm\ninotwo\; Z$	&   &      	& 15.03 & 14.45 & 14.21 & 14.21 & 14.16 & 13.34 & 9.64 & 8.54 & 8.54 & 8.29 & 0.57 & 0.55\\ %A01
wino $\chinoonepm\ninotwo\; h$	& 	&		& 15.03 & 14.29 & 13.99 & 13.99 & 13.88 & 12.97 & 9.08 & 8.50 & 8.50 & 8.38 & 0.57 & 0.56\\ %A02
slepton/sneutrino				&	& 	    & 1.83 	& 1.74 & 1.70  & 1.70 & 1.70 & 1.66  & 1.44  & 1.38 & 1.38 & 1.33   & 0.75 & 0.73\\
gluino 					& 1500  & 1100  & 512.27 &485.45 & 469.15 & 468.68 & 463.25 & 424.27 & 263.86 & 260.89 & 260.89  & 260.89 & 0.51 & 0.51 \\ %A05
%
 \bottomrule
\end{tabular}
\caption{Cutflow event yields in regions SR0A and SR0B for RPV models with the $\lambda_{12k}\neq 0$ coupling.
All yields correspond to weighted events, so that effects from lepton reconstruction efficiencies, trigger corrections, pileup reweighting, etc., are included.
They are normalized to the integrated luminosity of the data sample, $\int dt\;  L = 36.1~\mathrm{fb}^{-1}$.
The ``Initial'' number indicates the weighted number of events before any selection cut is applied. The last entries show the normalized number of events surviving the selection requirements
of SR0A and SR0B.
}
\label{tb:cutflow_weighted_sr0b}
}\end{table}


% @ 400 GeV  
% xsec = 0.0887325
% genEFF 
% ZZ: 0.011344
% Zh: 0.101610
\begin{table}[h]{\tiny \centering
\begin{tabular}{ccc | ccc ccc ccc cc  | cc}
\toprule
Model
& \rotatebox[origin=c]{90}{$m_\mathrm{NLSP}$ ~$[\GeV]$}
& \rotatebox[origin=c]{90}{BR($\ninoone \ra Z + \gravino\;(\%)$)}
%
& \rotatebox[origin=c]{90}{Initial}
& \rotatebox[origin=c]{90}{Generator Filter}
%
& \rotatebox[origin=c]{90}{Trigger} 
& \rotatebox[origin=c]{90}{Event Cleaning}
& \rotatebox[origin=c]{90}{$N_{e/\mu}  \geq 1$}
& \rotatebox[origin=c]{90}{$N_{e/\mu} = 2$}
& \rotatebox[origin=c]{90}{$N_{e/\mu} = 3$}
& \rotatebox[origin=c]{90}{$N_{e/\mu} = 4$}
& \rotatebox[origin=c]{90}{$ZZ$ selection}
& \rotatebox[origin=c]{90}{$E_{T}^{\mathrm{miss}} > 50~\mathrm{GeV}$ (SR0C)}
& \rotatebox[origin=c]{90}{$E_{T}^{\mathrm{miss}} > 100~\mathrm{GeV}$ (SR0D)}
%
& \rotatebox[origin=c]{90}{Efficiency SR0C} 
& \rotatebox[origin=c]{90}{Efficiency SR0D} \\
\hline
 %
GGM higgsino & 400 & 100 & 3203.45 & 36.34 & 28.77 & 27.64  & 26.14  & 23.34 & 14.19 & 7.59 & 5.71 & 5.44 & 4.84 & 0.002 & 0.002 \\
			 & 	   & 50	 & 3203.23 & 325.48 & 137.55 & 132.32 & 107.72 & 74.47 & 16.56  & 3.03 & 1.33  & 1.26 & 1.11 &  0.0004	& 0.0003 \\
 \bottomrule
\end{tabular}
\caption{
Cutflow event yields in regions SR0C and SR0D for higgsino GGM RPC model 
 with BR($\ninoone \ra Z + \gravino$) = 100\% (upper row) and 50\% (lower row), and $\chinoonepm/\ninotwo$ mass of $400~\GeV$. 
 All yields correspond to weighted events, so that effects from lepton reconstruction efficiencies, trigger corrections, pileup reweighting, etc., are included.
They are normalized to the integrated luminosity of the data sample, $\int dt\; L = 36.1~\mathrm{fb}^{-1}$.
The ``Initial'' number indicates the weighted number of events before any selection cut is applied. 
%
The ``Generator Filter'' step is applied during the MC generation of the simulated events; 
the BR=100\% sample has a generator filter of $\geq 4 e/\mu$ leptons with $p_T>4$~GeV and $|\eta|<2.8$, and 
the BR=50\% sample has a generator filter of $\geq 3 e/\mu/\tauhad$ leptons with $|\eta|<2.8$ and $p_T(e,\,\mu)>4$~GeV and $p_T(\tauhad^{\text{visible}})>15$~ GeV.
%
The $ZZ$ selection cutflow step refers to the mass window cut for the leading and subleading $Z$ boson
candidate between $81.2-101.2~\mathrm{GeV}$ and $61.2-101.2~\mathrm{GeV}$, respectively.
%
The last entries show the efficiency of events surviving the selection requirements defined in SR0C and SR0D.
}
\label{tb:cutflow_weighted_srcd}
}\end{table}


%\subsection{Cutflows SR1}
\begin{table}[h]{\tiny \centering
\begin{tabular}{lcc | ccc ccc ccc |c}
\toprule
Model 
& $m_\mathrm{NLSP}$ 
& $m_\mathrm{LSP}$ 
%
& \rotatebox[origin=c]{90}{Initial}
%
& \rotatebox[origin=c]{90}{Trigger} 
& \rotatebox[origin=c]{90}{Good Event} 
& \rotatebox[origin=c]{90}{$N_{e/\mu}  \geq 1$} 
& \rotatebox[origin=c]{90}{$N_{e/\mu} \geq 2$} 
& \rotatebox[origin=c]{90}{$N_{e/\mu} = 3$} 
&\rotatebox[origin=c]{90}{ Z veto} 
& \rotatebox[origin=c]{90}{$N_{\tauhad} \geq 1$ }
& \rotatebox[origin=c]{90}{$m_{\text{eff}} > 700$~GeV }
& \rotatebox[origin=c]{90}{Efficiency SR1} 
\\
\hline
 % new = Feb. 2018
 wino $\chinoonep\chinoonem$ 	& 800 & 400		& 79.85  & 73.87 & 70.61 & 67.48 & 46.56 & 14.60 & 13.53 & 6.73 & 6.18 & 0.08\\ %B01
 wino $\chinoonepm\ninotwo\; Z$	&     &      	& 171.79 & 157.05 & 149.97 & 142.36 & 93.88 & 27.00 & 21.78 & 10.12& 9.12 & 0.05\\ %B04
 wino $\chinoonepm\ninotwo\; H$	&     &		    & 171.79 & 157.88 & 149.42 & 140.40 & 89.45 & 25.29 & 22.79 & 10.92 & 10.13& 0.06 \\% B05%
slepton/sneutrino 				& 800 & 300 		& 24.65 & 24.41  & 23.18  & 22.62 & 17.94 & 6.63 & 6.29 & 3.49 & 3.27 & 0.13\\
 gluino 						& 1000 & 500    & 11746.51 & 10278.68 & 9733.46 & 8830.04 & 3520.69 & 3448.06 & 1642.80 & 273.58 & 273.58 & 0.02\\
%
 \bottomrule
\end{tabular}
\caption{Cutflow event yields in region SR1 for RPV models with the $\lambda_{i33}\neq0$ coupling.
All yields correspond to weighted events, so that effects from lepton reconstruction efficiencies, trigger corrections, pileup reweighting, etc., are included.
They are normalized to the integrated luminosity of the data sample, $\int dt\;  L = 36.1~\mathrm{fb}^{-1}$.
The ``Initial'' number indicates the weighted number of events before any selection cut is applied. The last entries show the normalized number of events surviving the selection requirements
of SR1.
}
\label{tb:cutflow_weighted_sr1}
}\end{table} 


%\subsection{Cutflows SR2}

\begin{table}[h]{\tiny \centering
\begin{tabular}{lcc | ccc ccc ccc | c}
\toprule
Model 
& \rotatebox[origin=c]{90}{$m_\mathrm{NLSP}$ ~$[\GeV]$}
& \rotatebox[origin=c]{90}{$m_\mathrm{LSP}$ ~$[\GeV]$}
%
& \rotatebox[origin=c]{90}{Initial} 
%
& \rotatebox[origin=c]{90}{Trigger} 
& \rotatebox[origin=c]{90}{Event Cleaning} 
& \rotatebox[origin=c]{90}{$N_{e/\mu}  \geq 1$} 
& \rotatebox[origin=c]{90}{$N_{e/\mu} = 2$} 
& \rotatebox[origin=c]{90}{Z veto } 
& \rotatebox[origin=c]{90}{$N_{\tauhad} \geq 1$} 
& \rotatebox[origin=c]{90}{$N_{\tauhad} \geq 2$} 
& \rotatebox[origin=c]{90}{$m_{\text{eff}} > 650$~GeV} 
& \rotatebox[origin=c]{90}{Efficiency SR2} 
\\
 \hline
 %
 wino $\chinoonep\chinoonem$ 	& 800 & 400  	& 79.85  & 73.87 &  70.61 & 67.48 & 27.19 & 26.45  & 16.16 & 4.87 & 4.61 & 0.06 \\ %C04
 wino $\chinoonepm\ninotwo\; Z$	&     &		& 171.79 & 157.05 & 149.97 & 142.36 & 57.55 & 55.65 & 31.56 & 7.64 & 7.19 & 0.04\\ %C02
 wino $\chinoonepm\ninotwo\; H$ &     &   	& 171.79 & 157.88 & 149.42 & 140.40 & 56.58 & 55.32 & 31.98 & 8.88 & 8.65 &0.05 \\ %C03
slepton/sneutrino  				& 800 & 300  & 24.65 & 24.41 & 23.18  & 22.62 & 8.38 & 8.29 & 5.25 & 1.93 & 1.81 & 0.07\\
gluino 				&1000 & 500     & 11746.51 & 10278.68 & 9733.46 & 8830.04 & 3520.69 & 3448.06 & 1642.80 & 273.58 & 273.58 & 0.02 \\
%
 \bottomrule
\end{tabular}
\caption{Cutflow event yields in region SR2 for RPV models with the $\lambda_{i33}\neq0$ coupling.
All yields correspond to weighted events, so that effects from lepton reconstruction efficiencies, trigger corrections, pileup reweighting, etc., are included.
They are normalized to the integrated luminosity of the data sample, $\int dt\;  L = 36.1~\mathrm{fb}^{-1}$.
The ``Initial'' number indicates the weighted number of events before any selection cut is applied. The last entries show the normalized number of events surviving the selection requirements
of SR2.
%
}
\label{tb:cutflow_weighted_sr2}
}\end{table} 




%\subsection{Slepton cross section}
\begin{center}
\begin{table}[h]{\centering
\begin{tabular}{cc}
\toprule
$m_\mathrm{NLSP}$ ~$[\GeV]$  & $\sigma(\mathrm{fb})$\\
\hline
400&	21.52\\
600&	3.205\\
800&	0.6828\\
900&	0.3409\\
\bottomrule
\end{tabular}
\caption{Cross sections for the $\sleptonL/\snu$ model for different NLSP masses.}
\label{tb:slep_xsec}
}\end{table} 
\end{center}

\FloatBarrier

